A Visual Formalism for Interacting Systems

Interacting systems are increasingly common. Many examples pervade our everyday lives: automobiles, aircraft, defense systems, telephone switching systems, financial systems, national governments, and so on. Closer to computer science, embedded systems and Systems of Systems are further examples of interacting systems. Common to all of these is that some "whole" is made up of constituent parts, and these parts interact with each other. By design, these interactions are intentional, but it is the unintended interactions that are problematic. The Systems of Systems literature uses the terms "constituent systems" and "constituents" to refer to systems that interact with each other. That practice is followed here. This paper presents a visual formalism, Swim Lane Event-Driven Petri Nets, that is proposed as a basis for Model-Based Testing (MBT) of interacting systems. In the absence of available tools, this model can only support the offline form of Model-Based Testing.

==> eptcsdata.tex <==
\providecommand{\firstpage}{41}
\providecommand{\publicationstatus}{A.K. Petrenko, B.-H. Schlingloff, N. Pakulin (Eds.):\\
Tenth Workshop on Model-Based Testing (MBT 2015)\\
EPTCS 180, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.180.3}{10.4204/EPTCS.180.3}}
\pdfoutput=1

